Hinged Truchet tiling fractals

This article describes a new method of producing space filling fractal dragon curves based on a hinged tiling procedure. The fractals produced can be generated by a simple L-system. The construction as a hinged tiling has the advantage of automatically implying that the fractiles produced tessellate, and that the Heighway fractal dragon curve, and the other curves constructed by this method, do not cross themselves. This also gives a new limiting procedure to apply to certain Truchet tilings. I include the computation of the fractal dimension of the boundary of one of the curves, and describe an algorithm for computing the sim value of the fractal boundary of these curves. The curves produced are well known. The hinged tiling approach is new, as is the algorithm for computing the sim value.

==> 001B27septD3.tex <==
\begin{scope}[rotate={0}]
\begin{scope}[shift={(-199.99999999999997,199.99999999999994)}]

  \begin{scope}[rotate={180}]
\begin{scope}[shift={(,0)}]
\draw[blue, opacity=0.25, line width=4mm] (0,0) -- ++(0,20.000000) 
-- ++(-20,0.000000) -- ++(0,-20.000000) -- ++(-20,0.000000) ;
\end{scope}
\end{scope}

  \foreach \i/\j/\l in {-5/90/brown,
    -15/90/brown,
   -5/-90/violet,
-15/-90/violet}{    
\begin{scope}[shift = {(0,\i)}  ]
\begin{scope}[rotate= {\j}]
  \begin{scope}[line width=0.05mm,scale=0.125]
    \bitC{\l}
  \end{scope}
    \end{scope}
\end{scope}
  }

  \foreach \i/\j/\k/\l in {30/-10/45/red,
    10/-30/45/red,
30/-10/-135/orange}{
\begin{scope}[shift = {(\i,\j)}  ]
\begin{scope}[rotate= {\k}]
  \begin{scope}[line width=0.1mm,scale=0.35355]
    \bitC{\l}
  \end{scope}
    \end{scope}
\end{scope}
}

  \foreach \i/\j/\k/\l in {1.25/-21.25/-45/cyan,
    3.75/-23.75/-45/cyan,
    6.25/-26.25/-45/cyan,
    8.75/-28.75/-45/cyan,
        6.25/-26.25/135/green,
        8.75/-28.75/135/green,    
    3.75/-23.75/135/green,
  1.25/-21.25/135/green}{
\begin{scope}[shift = {(\i,\j)}  ]
\begin{scope}[rotate= {\k}]
  \begin{scope}[line width=0.01mm,scale=0.0441941]
    \bitC{\l}
  \end{scope}
    \end{scope}
\end{scope}
}
  
  
    
\end{scope}
\end{scope}


==> 4times001.tex <==
\begin{scope}[rotate={-135}]
\begin{scope}[shift={(1.7763568394002505e-14,-282.84271247461885)}]
\filldraw[red] (0,0) circle (0.1);
\draw[yellow!70!gray] (0,0) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) 
-- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(-0.883883,0.000000) -- ++(0,0.883883) -- ++(-0.883883,0.000000) -- ++(0,-0.883883) -- ++(0.883883,0.000000) -- ++(0,-0.883883) ;
\end{scope}
\end{scope}


==> QQQ.tex <==
\begin{scope}[rotate={90}]
\begin{scope}[shift={(199.9999999999999,199.9999999999999)}]
\draw[red] (0,0) -- ++(0,-2.500000) 
-- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) 
-- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) 
-- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(-2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,-2.500000) -- ++(-2.5,0.000000) -- ++(0,-2.500000) -- ++(2.5,0.000000) -- ++(0,2.500000) -- ++(2.5,0.000000) ;
\end{scope}
\end{scope}



==> manypartsA3.tex <==
\newcommand\bitB[9]{
\begin{scope}[shift={(200,-200)}]
  \begin{scope}[rotate={-135}]
\begin{scope}[shift={(0,-282.84271247461885)}]
  \begin{scope}[rotate={-135}]
\draw[line width = 0.5,#1] (0,0) -- ++(0,-2.5) 
-- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;
\draw[line width = 0.5,#1] (-20,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) ;
\draw[line width = 0.5,#1] (-20,-20) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) 
-- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) ;
\draw[line width = 0.5,#1] (0,-20) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) 
-- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) ;
\draw[line width = 0.5,#1] (0,-40) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) 
-- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;
\draw[line width = 0.5,#1] (-20,-40) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) 
-- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;
\draw[line width = 0.5,#1] (-20,-20) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;
\draw[line width = 0.5,#1] (-40,-20) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;
\draw[line width = 0.5,#1] (-40,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) 
-- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) ;
\draw[line width = 0.5,#1] (-20,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) ;

\draw[line width = 0.5,#1] (0,20) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) 
-- ++(2.5,0) -- ++(0,2.5) -- ++(-2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,-2.5) -- ++(-2.5,0) -- ++(0,-2.5) -- ++(2.5,0) -- ++(0,2.5) -- ++(2.5,0) ;
\end{scope}
\end{scope}
  \end{scope}
  \end{scope}
}


\newcommand\bitC[1]{
\bitB{#1}{#1}{#1}{#1}{#1}{#1}{#1}{#1}{#1}
  }

